Faster Motion Planning via Restarts

Randomized methods such as PRM and RRT are widely used in motion planning. However, in some cases, their running-time suffers from inherent instability, leading to ``catastrophic'' performance even for relatively simple instances. We apply stochastic restart techniques, some of them new, for speeding up Las Vegas algorithms, that provide dramatic speedups in practice (a factor of $3$ [or larger] in many cases). Our experiments demonstrate that the new algorithms have faster runtimes, shorter paths, and greater gains from multi-threading (when compared with straightforward parallel implementation). We prove the optimality of the new variants. Our implementation is open source, available on github, and is easy to deploy and use.

==> figs/bug_len_2_7713.tex <==
\begin{tabular}{|l||r|r|r||r|r||r|r|r|}
  \hline
  \textbf{Simulation} & \textbf{\#} & \textbf{Succs} & \textbf{Fails} & \textbf{Mean} & \textbf{Median} & \textbf{Std Dev} & \textbf{Min} & \textbf{Max} \\\hline
  \cellcolor{lightgray}{\texttt{Parallel}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{36}} & \cellcolor{lightgray}{\FailX{64}} & \cellcolor{lightgray}{\texttt{1526.69}} & \cellcolor{lightgray}{\texttt{1427.50}} & \cellcolor{lightgray}{\texttt{904.55}} & \cellcolor{lightgray}{\texttt{6.00}} & \cellcolor{lightgray}{\texttt{2925.00}} \\
\hline
  \texttt{Wide} & \texttt{100} & \texttt{68} & \FailX{32} & \texttt{787.65} & \texttt{503.00} & \texttt{826.54} & \texttt{5.00} & \texttt{2899.00} \\
  \cellcolor{lightgray}{\texttt{Random}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{0}} & \cellcolor{lightgray}{\texttt{446.01}} & \cellcolor{lightgray}{\texttt{209.50}} & \cellcolor{lightgray}{\texttt{543.65}} & \cellcolor{lightgray}{\texttt{6.00}} & \cellcolor{lightgray}{\texttt{2519.00}} \\
  \texttt{Counter+Cache} & \texttt{100} & \texttt{100} & \texttt{0} & \texttt{346.37} & \texttt{223.50} & \texttt{349.84} & \texttt{5.00} & \texttt{2084.00} \\
  \cellcolor{lightgray}{\texttt{Counter}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{0}} & \cellcolor{lightgray}{\texttt{315.14}} & \cellcolor{lightgray}{\texttt{190.50}} & \cellcolor{lightgray}{\texttt{325.23}} & \cellcolor{lightgray}{\texttt{5.00}} & \cellcolor{lightgray}{\texttt{1755.00}} \\
  \texttt{Random $\zeta(2)$} & \texttt{100} & \texttt{100} & \texttt{0} & \texttt{275.54} & \texttt{155.50} & \texttt{303.83} & \texttt{5.00} & \texttt{1392.00} \\\hline
\end{tabular}


==> figs/bug_len_2_valis.tex <==
\begin{tabular}{|l||r|r|r||r|r||r|r|r|}
  \hline
  \textbf{Simulation} & \textbf{\#} & \textbf{Succs} & \textbf{Fails} & \textbf{Mean} & \textbf{Median} & \textbf{Std Dev} & \textbf{Min} & \textbf{Max} \\\hline
  \cellcolor{lightgray}{\texttt{Parallel}} & \cellcolor{lightgray}{\texttt{61}} & \cellcolor{lightgray}{\texttt{0}} & \cellcolor{lightgray}{\FailX{61}} & \cellcolor{lightgray}{\texttt{---}} & \cellcolor{lightgray}{\texttt{---}} & \cellcolor{lightgray}{\texttt{---}} & \cellcolor{lightgray}{\texttt{---}} & \cellcolor{lightgray}{\texttt{---}} \\
\hline
  \texttt{Counter+Cache} & \texttt{100} & \texttt{57} & \FailX{43} & \texttt{852.95} & \texttt{602.00} & \texttt{763.67} & \texttt{12.00} & \texttt{2994.00} \\
  \cellcolor{lightgray}{\texttt{Counter}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{61}} & \cellcolor{lightgray}{\FailX{39}} & \cellcolor{lightgray}{\texttt{1148.41}} & \cellcolor{lightgray}{\texttt{966.00}} & \cellcolor{lightgray}{\texttt{933.65}} & \cellcolor{lightgray}{\texttt{11.00}} & \cellcolor{lightgray}{\texttt{2865.00}} \\
  \texttt{Random $\zeta(2)$} & \texttt{100} & \texttt{62} & \FailX{38} & \texttt{1155.65} & \texttt{967.00} & \texttt{920.35} & \texttt{3.00} & \texttt{2946.00} \\\hline
\end{tabular}


==> figs/maze_7713.tex <==
\begin{tabular}{|l||r||r|r||r|r|r|}
  \hline
  \textbf{Simulation} & \textbf{\#} & \textbf{Mean} & \textbf{Median} & \textbf{Std Dev} & \textbf{Min} & \textbf{Max} \\\hline
  \cellcolor{lightgray}{\texttt{Parallel}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{98.23}} & \cellcolor{lightgray}{\texttt{101.00}} & \cellcolor{lightgray}{\texttt{8.68}} & \cellcolor{lightgray}{\texttt{76.00}} & \cellcolor{lightgray}{\texttt{114.00}} \\
\hline
  \texttt{Wide} & \texttt{100} & \texttt{150.18} & \texttt{150.00} & \texttt{17.42} & \texttt{105.00} & \texttt{193.00} \\
  \cellcolor{lightgray}{\texttt{Counter}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{145.18}} & \cellcolor{lightgray}{\texttt{143.50}} & \cellcolor{lightgray}{\texttt{21.36}} & \cellcolor{lightgray}{\texttt{102.00}} & \cellcolor{lightgray}{\texttt{191.00}} \\
  \texttt{Random $\zeta(2)$} & \texttt{100} & \texttt{137.82} & \texttt{135.50} & \texttt{26.55} & \texttt{86.00} & \texttt{227.00} \\
  \cellcolor{lightgray}{\texttt{Counter+Cache}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{135.66}} & \cellcolor{lightgray}{\texttt{132.00}} & \cellcolor{lightgray}{\texttt{20.59}} & \cellcolor{lightgray}{\texttt{95.00}} & \cellcolor{lightgray}{\texttt{211.00}} \\\hline
\end{tabular}


==> figs/maze_valis.tex <==
\begin{tabular}{|l||r||r|r||r|r|r|}
  \hline
  \textbf{Simulation} & \textbf{\#} & \textbf{Mean} & \textbf{Median} & \textbf{Std Dev} & \textbf{Min} & \textbf{Max} \\\hline
  \cellcolor{lightgray}{\texttt{Parallel}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{124.77}} & \cellcolor{lightgray}{\texttt{124.00}} & \cellcolor{lightgray}{\texttt{19.82}} & \cellcolor{lightgray}{\texttt{85.00}} & \cellcolor{lightgray}{\texttt{183.00}} \\
\hline
  \texttt{Counter} & \texttt{100} & \texttt{318.64} & \texttt{324.00} & \texttt{82.94} & \texttt{173.00} & \texttt{562.00} \\
  \cellcolor{lightgray}{\texttt{Random $\zeta(2)$}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{247.45}} & \cellcolor{lightgray}{\texttt{221.00}} & \cellcolor{lightgray}{\texttt{113.12}} & \cellcolor{lightgray}{\texttt{86.00}} & \cellcolor{lightgray}{\texttt{901.00}} \\
  \texttt{Counter+Cache} & \texttt{100} & \texttt{220.96} & \texttt{225.00} & \texttt{48.79} & \texttt{120.00} & \texttt{325.00} \\
  \cellcolor{lightgray}{\texttt{Random}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{214.43}} & \cellcolor{lightgray}{\texttt{194.50}} & \cellcolor{lightgray}{\texttt{93.33}} & \cellcolor{lightgray}{\texttt{95.00}} & \cellcolor{lightgray}{\texttt{542.00}} \\
  \texttt{Wide} & \texttt{100} & \texttt{165.01} & \texttt{157.00} & \texttt{36.40} & \texttt{96.00} & \texttt{286.00} \\\hline
\end{tabular}


==> figs/path_lengths.tex <==
\begin{tabular}{|l||r||r|r||r|r|r|}
  \cline{3-7}
  \multicolumn{2}{c||}{}
  &\multicolumn{5}{c|}{Path lengths}
  \\
  \hline
  \textbf{Simulation} & \textbf{\#} & \textbf{Mean} & \textbf{Median} & \textbf{Std Dev} & \textbf{Min} & \textbf{Max} \\\hline
  \cellcolor{lightgray}{\texttt{Parallel}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{208.30}} & \cellcolor{lightgray}{\texttt{232.12}} & \cellcolor{lightgray}{\texttt{68.69}} & \cellcolor{lightgray}{\texttt{23.78}} & \cellcolor{lightgray}{\texttt{258.97}} \\
  \texttt{Random} & \texttt{100} & \texttt{148.53} & \texttt{226.89} & \texttt{100.20} & \texttt{22.47} & \texttt{249.52} \\
  \cellcolor{lightgray}{\texttt{Random $\zeta(2)$}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{148.18}} & \cellcolor{lightgray}{\texttt{226.34}} & \cellcolor{lightgray}{\texttt{99.37}} & \cellcolor{lightgray}{\texttt{24.50}} & \cellcolor{lightgray}{\texttt{255.39}} \\
  \texttt{Counter} & \texttt{100} & \texttt{127.58} & \texttt{45.71} & \texttt{100.08} & \texttt{21.63} & \texttt{249.36} \\\hline
\end{tabular}


==> figs/shelves_7713.tex <==
\begin{tabular}{|l||r||r|r||r|r|r|}
  \hline
  \textbf{Simulation} & \textbf{\#} & \textbf{Mean} & \textbf{Median} & \textbf{Std Dev} & \textbf{Min} & \textbf{Max} \\\hline
  \cellcolor{lightgray}{\texttt{Parallel}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{154.97}} & \cellcolor{lightgray}{\texttt{39.50}} & \cellcolor{lightgray}{\texttt{271.33}} & \cellcolor{lightgray}{\texttt{5.00}} & \cellcolor{lightgray}{\texttt{1400.00}} \\
\hline
  \texttt{Wide} & \texttt{100} & \texttt{115.64} & \texttt{61.00} & \texttt{159.18} & \texttt{4.00} & \texttt{1096.00} \\
  \cellcolor{lightgray}{\texttt{Random $\zeta(2)$}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{64.69}} & \cellcolor{lightgray}{\texttt{41.50}} & \cellcolor{lightgray}{\texttt{68.92}} & \cellcolor{lightgray}{\texttt{5.00}} & \cellcolor{lightgray}{\texttt{315.00}} \\
  \texttt{Counter+Cache} & \texttt{100} & \texttt{64.33} & \texttt{53.00} & \texttt{61.56} & \texttt{4.00} & \texttt{364.00} \\
  \cellcolor{lightgray}{\texttt{Counter}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{58.42}} & \cellcolor{lightgray}{\texttt{39.00}} & \cellcolor{lightgray}{\texttt{53.90}} & \cellcolor{lightgray}{\texttt{5.00}} & \cellcolor{lightgray}{\texttt{234.00}} \\
  \texttt{Random} & \texttt{100} & \texttt{47.54} & \texttt{27.00} & \texttt{59.79} & \texttt{4.00} & \texttt{442.00} \\
\hline
  \cellcolor{lightgray}{\texttt{\TTL $2$}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{51.76}} & \cellcolor{lightgray}{\texttt{38.00}} & \cellcolor{lightgray}{\texttt{50.23}} & \cellcolor{lightgray}{\texttt{4.00}} & \cellcolor{lightgray}{\texttt{237.00}} \\
  \texttt{\TTL $3$} & \texttt{100} & \texttt{47.94} & \texttt{27.00} & \texttt{49.57} & \texttt{5.00} & \texttt{200.00} \\
  \cellcolor{lightgray}{\texttt{\TTL $5$}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{50.51}} & \cellcolor{lightgray}{\texttt{34.00}} & \cellcolor{lightgray}{\texttt{56.48}} & \cellcolor{lightgray}{\texttt{4.00}} & \cellcolor{lightgray}{\texttt{303.00}} \\
  \texttt{\TTL $10$} & \texttt{100} & \texttt{53.13} & \texttt{38.50} & \texttt{46.54} & \texttt{5.00} & \texttt{272.00} \\\hline
\end{tabular}


==> figs/shelves_catapult.tex <==
\begin{tabular}{|l||r|r|r||r|r||r|r|r|r}
  \hline
  \textbf{Simulation} & \textbf{\#} & \textbf{Succs} & \textbf{Fails} & \textbf{Mean} & \textbf{Median} & \textbf{Std Dev} & \textbf{Min} & \textbf{Max} \\\hline
  \cellcolor{lightgray}{\texttt{Single}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{7}} & \cellcolor{lightgray}{\FailX{93}} & \cellcolor{lightgray}{\texttt{898.14}} & \cellcolor{lightgray}{\texttt{312.00}} & \cellcolor{lightgray}{\texttt{1074.23}} & \cellcolor{lightgray}{\texttt{34.00}} & \cellcolor{lightgray}{\texttt{2956.00}} \\
\hline
  \texttt{Random $\zeta(2)$} & \texttt{100} & \texttt{19} & \FailX{81} & \texttt{1199.63} & \texttt{907.00} & \texttt{1034.27} & \texttt{2.00} & \texttt{2933.00} \\
  \cellcolor{lightgray}{\texttt{Random}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{30}} & \cellcolor{lightgray}{\FailX{70}} & \cellcolor{lightgray}{\texttt{1535.50}} & \cellcolor{lightgray}{\texttt{1527.00}} & \cellcolor{lightgray}{\texttt{749.81}} & \cellcolor{lightgray}{\texttt{149.00}} & \cellcolor{lightgray}{\texttt{2987.00}} \\
  \texttt{Counter} & \texttt{100} & \texttt{37} & \FailX{63} & \texttt{1208.51} & \texttt{1171.00} & \texttt{814.20} & \texttt{18.00} & \texttt{2768.00} \\
  \cellcolor{lightgray}{\texttt{Wide}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{40}} & \cellcolor{lightgray}{\FailX{60}} & \cellcolor{lightgray}{\texttt{1422.03}} & \cellcolor{lightgray}{\texttt{1431.50}} & \cellcolor{lightgray}{\texttt{753.52}} & \cellcolor{lightgray}{\texttt{88.00}} & \cellcolor{lightgray}{\texttt{2967.00}} \\
  \texttt{Counter+Cache} & \texttt{100} & \texttt{45} & \FailX{55} & \texttt{1362.18} & \texttt{1219.00} & \texttt{861.28} & \texttt{3.00} & \texttt{2849.00} \\\hline
\end{tabular}


==> figs/shelves_valis.tex <==
\begin{tabular}{|l||r|r|r||r|r||r|r|r|r}
  \hline
  \textbf{Simulation} & \textbf{\#} & \textbf{Succs} & \textbf{Fails} & \textbf{Mean} & \textbf{Median} & \textbf{Std Dev} & \textbf{Min} & \textbf{Max} \\\hline
  \cellcolor{lightgray}{\texttt{Parallel}} & \cellcolor{lightgray}{\texttt{42}} & \cellcolor{lightgray}{\texttt{25}} & \cellcolor{lightgray}{\FailX{17}} & \cellcolor{lightgray}{\texttt{733.44}} & \cellcolor{lightgray}{\texttt{458.00}} & \cellcolor{lightgray}{\texttt{632.32}} & \cellcolor{lightgray}{\texttt{46.00}} & \cellcolor{lightgray}{\texttt{2220.00}} \\
  \texttt{Wide} & \texttt{100} & \texttt{99} & \FailX{1} & \texttt{606.43} & \texttt{398.00} & \texttt{657.69} & \texttt{1.00} & \texttt{2972.00} \\
\hline
  \cellcolor{lightgray}{\texttt{Random}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{0}} & \cellcolor{lightgray}{\texttt{541.49}} & \cellcolor{lightgray}{\texttt{365.50}} & \cellcolor{lightgray}{\texttt{513.54}} & \cellcolor{lightgray}{\texttt{3.00}} & \cellcolor{lightgray}{\texttt{2283.00}} \\
  \texttt{Random $\zeta(2)$} & \texttt{100} & \texttt{99} & \FailX{1} & \texttt{477.57} & \texttt{308.00} & \texttt{486.30} & \texttt{1.00} & \texttt{1954.00} \\
  \cellcolor{lightgray}{\texttt{Counter}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{0}} & \cellcolor{lightgray}{\texttt{462.92}} & \cellcolor{lightgray}{\texttt{268.00}} & \cellcolor{lightgray}{\texttt{549.91}} & \cellcolor{lightgray}{\texttt{3.00}} & \cellcolor{lightgray}{\texttt{2802.00}} \\
  \texttt{Counter+Cache} & \texttt{100} & \texttt{100} & \texttt{0} & \texttt{368.49} & \texttt{284.00} & \texttt{333.42} & \texttt{7.00} & \texttt{2168.00} \\\hline
\end{tabular}


==> figs/simple_passage_valis.tex <==
\begin{tabular}{|l||r|r|r||r|r||r|r|r|}
  \hline
  \textbf{Simulation} & \textbf{\#} & \textbf{Succs} & \textbf{Fails} & \textbf{Mean} & \textbf{Median} & \textbf{Std Dev} & \textbf{Min} & \textbf{Max} \\\hline
  \cellcolor{lightgray}{\texttt{Single}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{67}} & \cellcolor{lightgray}{\FailX{33}} & \cellcolor{lightgray}{\texttt{840.82}} & \cellcolor{lightgray}{\texttt{637.00}} & \cellcolor{lightgray}{\texttt{770.50}} & \cellcolor{lightgray}{\texttt{1.00}} & \cellcolor{lightgray}{\texttt{2963.00}} \\
  \texttt{Parallel} & \texttt{100} & \texttt{100} & \texttt{0} & \texttt{117.49} & \texttt{26.50} & \texttt{234.22} & \texttt{1.00} & \texttt{1509.00} \\
\hline
  \cellcolor{lightgray}{\texttt{Wide}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{0}} & \cellcolor{lightgray}{\texttt{24.93}} & \cellcolor{lightgray}{\texttt{16.00}} & \cellcolor{lightgray}{\texttt{29.83}} & \cellcolor{lightgray}{\texttt{1.00}} & \cellcolor{lightgray}{\texttt{145.00}} \\
  \texttt{Random} & \texttt{100} & \texttt{100} & \texttt{0} & \texttt{20.10} & \texttt{12.50} & \texttt{21.97} & \texttt{1.00} & \texttt{99.00} \\
  \cellcolor{lightgray}{\texttt{Counter+Cache}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{0}} & \cellcolor{lightgray}{\texttt{19.76}} & \cellcolor{lightgray}{\texttt{11.50}} & \cellcolor{lightgray}{\texttt{20.64}} & \cellcolor{lightgray}{\texttt{1.00}} & \cellcolor{lightgray}{\texttt{108.00}} \\
  \texttt{Random $\zeta(2)$} & \texttt{100} & \texttt{100} & \texttt{0} & \texttt{18.11} & \texttt{12.00} & \texttt{21.82} & \texttt{1.00} & \texttt{125.00} \\
  \cellcolor{lightgray}{\texttt{Counter}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{100}} & \cellcolor{lightgray}{\texttt{0}} & \cellcolor{lightgray}{\texttt{14.74}} & \cellcolor{lightgray}{\texttt{11.00}} & \cellcolor{lightgray}{\texttt{16.42}} & \cellcolor{lightgray}{\texttt{1.00}} & \cellcolor{lightgray}{\texttt{110.00}} \\\hline
\end{tabular}

